Spectroscopic Observations of Selected Planetary Nebulae from the HASH Database

We conducted research on the classification and physical properties of 10 objects from the HASH (Hong Kong/Australian Astronomical Observatory/Strasbourg Observatory H-alpha Planetary Nebula (PN)) database with small angular sizes (< 8\arcsec) in the northern hemisphere. The sample consisted of 6 Likely PNe, 2 new candidates, one emission-line star, and one object of unknown nature. Among them, we observed 4 objects for the first time using the medium-resolution TFOSC spectrograph located on the RTT150 cm of the T\"UB\.ITAK National Observatory (TUG). To investigate the classification of the observed objects, we utilized the emission line ratios of [O III]/H$_{\gamma}$, [O III]/H$_{\beta}$, [N II]/H$_{\alpha}$ and [S II]/H$_{\alpha}$ and diagnostic diagrams such as the Sabbadin-Minello-Bianchini (SMB) and Baldwin-Phillips-Terlevich (BPT). When considering a broader range of diagnostic criteria compared to those provided in the literature, our analyses resulted in the reclassification of 4 objects from Likely PNe to True PNe and the retention of the previous classification for the remaining 6 objects. In addition, we obtained various physical conditions such as electron temperatures, electron densities, logarithmic extinction coefficients, and excitation classes for the 10 objects under study. Our analysis revealed that the ionic abundances of the majority of these objects were in agreement with Galactic PNe. Our spectral observations have led to the updating of 10 PNe in the HASH database.

==> cover.tex <==
To whom it may concern,

In this manuscript, we focused on the classification of Planetary Nebulae (PNe). It covers 5 years of spectroscopic observations of PNe. The techniques are the detection of emission lines, emission line ratios, and diagnostic diagrams. Moreover, the Physical properties of the PNe are also discussed.

We would like to submit this manuscript for publication as a "Research Article" in Monthly Notices of the Royal Astronomical Society.

Yours Sincerely,
Nazım Aksaker
